On How Users Edit Computer-Generated Visual Stories

A significant body of research in Artificial Intelligence (AI) has focused on generating stories automatically, either based on prior story plots or input images. However, literature has little to say about how users would receive and use these stories. Given the quality of stories generated by modern AI algorithms, users will nearly inevitably have to edit these stories before putting them to real use. In this paper, we present the first analysis of how human users edit machine-generated stories. We obtained 962 short stories generated by one of the state-of-the-art visual storytelling models. For each story, we recruited five crowd workers from Amazon Mechanical Turk to edit it. Our analysis of these edits shows that, on average, users (i) slightly shortened machine-generated stories, (ii) increased lexical diversity in these stories, and (iii) often replaced nouns and their determiners/articles with pronouns. Our study provides a better understanding on how users receive and edit machine-generated stories,informing future researchers to create more usable and helpful story generation systems.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.


==> related_work.tex <==
We now review two general end-to-end approaches that apply deep neural networks: visual captioning (storytelling) and automatic post-editing. In addition, we discuss some work of machine assistant to emphasize our goal.  

\subsection{Stylized Visual Captioning and Storytelling}

\textit{StyleNet}, which uses an encoder-decoder based model for learning romantic and humorous captions~\cite{gan2017styleNet}. \textit{StyleNet} consists of a convolutional neural network (CNN) and many recurrent neural networks (RNN) that act as an encoder and decoders respectively. The CNN encodes images into a fixed-length vector, which represents a data point in a high dimensional space. The RNNs decode the vector into captions with various lengths and styles. The training data of \textit{StyleNet} includes paired images and factual-captions, together with unlabeled romantic-style and humorous-style text corpus. The decoders are trained by using multi-task learning (MTL), where the training phase alternates among several tasks~\cite{luong2015multi}. Training the main task (e.g., language-to-language machine translation) with several additional tasks (e.g., image captioning or unsupervised learning) jointly can increase the performance of the main task~\cite{luong2015multi}. However, those works only focus on several specific style, but our task is more diverse depends on what human edit, getting closer to what they are sharing on social media.     

\textit{SemStyle}~\cite{mathews2018semstyle}, which also adopted the encoder-decoder network. Both the encoder and decoder were trained separately on image caption datasets and a large text corpus respectively. The encoder mapped images to semantics terms, and the decoder converted semantics terms into sentences. Different from \textit{StyleNet} that took the latest output of the encoder as input for the decoder, \textit{SemStyle} added the attention mechanism. This idea is analogous to the attention mechanism in machine translation, which allows the decoder to access multiple outputs from the encoder, instead of using only the output from the final layer of the encoder~\cite{bahdanau2014neural,luong2015effective}. Even though\textit{SemStyle}~\cite{mathews2018semstyle} can add multiple different style through attention mechanism, they need large dataset for training. Our post-edit model only train on small part of VIST Dataset and we claim that it can also obtain significant improvement.   

\subsection{Machine Support Writing}
Nowadays, some works developed machine to support people designing creative work. Elizabeth et al. propose a machine-in-the-loop framework that assist people improving the writing ability\cite{clark2018creative}. Different from previous work, our task additionally use image-captioning model to let users edit the stories depends on their shared photos. 

\subsection{Neural Automatic Post-Editing}

Another approach is neural automatic post-editing (APE), which uses deep learning to automatically revises the text generated from a machine translation (MT) system, given both the source sentences and translated sentences. The MT is treated as a black-box system that is fixed and not modifiable. The goal of APE is to correct systematic MT errors, thereby reducing translators' workload and eventually increasing translation productivity~\cite{astudillo2018proceedings}. APE is different from computer-assisted post-editing, which aims to develop interactive systems that suggest modifications based on human guidance, such as~\cite{grangier2018quickedit,peris2017interactive}. Additionally, neural APE is sentence-to-sentence, which differs from previous state-of-the-art phrase-based models that translate and reorder phrase segments for each sentence, such as~\cite{simard2007statistical,bechara2011statistical}. 
  
The encoder-decoder model has been applied to automatic post-editing. For instance, Libovicky et al. developed a system with many encoders and a decoder~\cite{libovicky2016cuni}. The input of the encoders are pairs of original sentences and machine-translated sentences. The output of the decoder are post-edited sentences. To prevent the model from paraphrasing the original sentences instead of editing them, the post-edited sentences are represented as a sequence of edit operations: \textit{keep}, \textit{delete}, and \textit{insert}. Another system, proposed by Junczys-Dowmunt and Grundkiewicz, adopted an ensemble-based approach to combined multiple deep neural networks with a log-linear model~\cite{junczys2016log}. This approach enabled each component in the ensemble to take different inputs, including the post-edited and machine-translated sentences. The system overcame the problem of limited APE training data by generating a large amount of artificial training data with back-translation~\cite{sennrich2015improving}. The idea was to use two phase-based MT systems to translate German to English and then back to German. The original German, the translated English, and the back-translated German are treated as the post-edited, source, and the machine-translated sentences respectively. Model sophisticated sequence-to-sequence learning models with the attention mechanism that extended these two works were later proposed~\cite{junczys2017exploration,libovicky2017attention}.

Compare to those previous works, our APE generates text from user's personal photos which assist human sharing their daily life on social media. In addition, our work conduct human evaluation through Amazon Mechanical Turk which is more reliable for sharing on social media. 


